iFinder: Structured Zero-Shot Vision-Based LLM Grounding for Dash-Cam Video Reasoning

Grounding large language models (LLMs) in domain-specific tasks like post-hoc dash-cam driving video analysis is challenging due to their general-purpose training and lack of structured inductive biases. As vision is often the sole modality available for such analysis (i.e., no LiDAR, GPS, etc.), existing video-based vision-language models (V-VLMs) struggle with spatial reasoning, causal inference, and explainability of events in the input video. To this end, we introduce iFinder, a structured semantic grounding framework that decouples perception from reasoning by translating dash-cam videos into a hierarchical, interpretable data structure for LLMs. iFinder operates as a modular, training-free pipeline that employs pretrained vision models to extract critical cues -- object pose, lane positions, and object trajectories -- which are hierarchically organized into frame- and video-level structures. Combined with a three-block prompting strategy, it enables step-wise, grounded reasoning for the LLM to refine a peer V-VLM's outputs and provide accurate reasoning. Evaluations on four public dash-cam video benchmarks show that iFinder's proposed grounding with domain-specific cues, especially object orientation and global context, significantly outperforms end-to-end V-VLMs on four zero-shot driving benchmarks, with up to 39% gains in accident reasoning accuracy. By grounding LLMs with driving domain-specific representations, iFinder offers a zero-shot, interpretable, and reliable alternative to end-to-end V-VLMs for post-hoc driving video understanding.

==> figs/suppl_qual.tex <==
\begin{figure*}[!t]
    \centering\tiny
    \resizebox{\columnwidth}{!}{
    \setlength\tabcolsep{0.5pt}
    \begin{tabular}{p{0.24\linewidth} p{0.27\linewidth} p{0.24\linewidth} p{0.27\linewidth}} 
        \begin{minipage}{\linewidth}
            \begin{center}
                \raggedright\includegraphics[width=0.75\linewidth]{figs/images/examples/supp_qual_1}\\ 
                \textbf{Q:} \textit{Is there traffic in your lane? \newline If so, what types of vehicles are present?}?
                % ce3084593e16b501a27dbbef7b2aa653
            \end{center}
        \end{minipage} &
        \parbox{\linewidth}{ 
            \raggedright
            \scalebox{.75}{\textbf{GT:} Yes, a cyclist.}
            \includegraphics[scale=0.3]{figs/images/suppl_qua1_bubble.pdf}
        } &
        \begin{minipage}{\linewidth}
            \begin{center}
            \raggedright\includegraphics[width=0.75\linewidth]{figs/images/examples/supp_qual_2} \\
            \scalebox{.95}{\textbf{Q:} \textit{Is there a traffic light in sight?}}\newline\scalebox{.95}{\textit{If so, what color is it exhibiting?}}
                % 852232e46c71d346dcb9f223647c0970
            \end{center}
        \end{minipage} &
        \parbox{\linewidth}{ 
            \raggedright
            \scalebox{.75}{\textbf{GT:} Yes, green.}\\
            \includegraphics[scale=0.3]{figs/images/suppl_qua2_bubble.pdf}}
        \\
        \midrule
        \begin{minipage}{\linewidth}
            \begin{center}
            \raggedright\includegraphics[width=0.75\linewidth]{figs/images/examples/suppl_qual_3_43_002437_000048} \\
            \textbf{Q:} \textit{What is the cause of the accident?}
             % frame: 00048
            \end{center}
        \end{minipage} &
        \parbox{\linewidth}{ 
            \raggedright\scalebox{.7}{\textbf{GT:} The car does not notice the coming vehicles when crossing the road.}
            \includegraphics[scale=0.3]{figs/images/suppl_qua3_bubble.pdf}
        }
        &
        % MMAU dataset
        \begin{minipage}{\linewidth}
            \begin{center}
            \raggedright\includegraphics[width=0.75\linewidth]{figs/images/examples/suppl_qual_4_10_013746_000030.jpg} \\
            \textbf{Q:} \textit{What is the cause of the accident?}
                % frame: 00030
            \end{center}
        \end{minipage} &
        \parbox{\linewidth}{ 
            \raggedright\scalebox{.75}{\textbf{GT:} The car does not notice the coming vehicles when crossing the road.}
            \includegraphics[scale=0.3]{figs/images/suppl_qua4_bubble.pdf}
        }
    \end{tabular}

    
    }
    \caption{\textbf{Additional Qualitative comparison on LingoQA. Bottom row is Peer-correction.}}
    \label{fig:suppl_qual}
\end{figure*}
